Local Projections of Low-Momentum Potentials

Nuclear interactions evolved via renormalization group methods to lower resolution become increasingly non-local (off-diagonal in coordinate space) as they are softened. This inhibits both the development of intuition about the interactions and their use with some methods for solving the quantum many-body problem. By applying "local projections", a softened interaction can be reduced to a local effective interaction plus a non-local residual interaction. At the two-body level, a local projection after similarity renormalization group (SRG) evolution manifests the elimination of short-range repulsive cores and the flow toward universal low-momentum interactions. The SRG residual interaction is found to be relatively weak at low energy, which motivates a perturbative treatment.

==> v7_arxiv v1/macros.tex <==
% !TEX root = DeepBS.tex
% !TEX TS-program = LaTeXmk
% !TEX encoding = UTF-8 Unicode
% !TEX spellcheck = en_US


% Environment Shortcuts
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}


% List Shortcuts
\newcommand{\li}{\item}

% Reference Shortcuts
\newcommand{\fref}[1]{\ref{fig:#1}}

% Common Mathematical Operations
\newcommand{\comm}[2]{\ensuremath{[#1,#2]}}

% Bra and Ket notation
\newcommand{\bra}[1]{\ensuremath{\langle#1|}}
\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}
\newcommand{\Bra}[1]{\ensuremath{\left<#1\right|}}
\newcommand{\Ket}[1]{\ensuremath{\left|#1\right>}}
\newcommand{\braket}[2]{\ensuremath{\langle#1|#2\rangle}}
\newcommand{\braketOne}[1]{\ensuremath{\langle#1\rangle}}
\newcommand{\Braket}[2]{\ensuremath{\left<#1\middle|#2\right>}}

% SRG generators
\newcommand{\Hdiag}{\ensuremath{H_{d}}}  % or {\rm d}
\newcommand{\Trel}{\ensuremath{T_{\rm rel}}}

% Interactions
\newcommand{\vlowk}{\ensuremath{V_{{\rm low}\,k}}}
\newcommand{\vsrg}{\ensuremath{V_{\lambda}}}
\newcommand{\vbare}{\ensuremath{V_{\rm NN}}}
\newcommand{\vcut}{\ensuremath{V_{\flow,\Lambda}}}
\newcommand{\vnn}{\ensuremath{V_{\rm NN}}}

% Hamiltonian Components
\newcommand{\Hzero}{\ensuremath{T_{\rm rel}}}
\newcommand{\Hint}{\ensuremath{V}}

% Units
\newcommand{\fm}{\, \text{fm}}
\newcommand{\fmi}{\, \text{fm}^{-1}}
\newcommand{\mev}{\, \text{MeV}}

% Common Constructs (vectors for momenta, positions, flow parameters)
\newcommand{\flow}{\ensuremath{\lambda}}
\newcommand{\qvec}{\ensuremath{{\bf q}^{\protect\phantom{\prime}}}}
\newcommand{\kvec}{\ensuremath{{{\bf k}^{\protect\phantom{\prime}}}}}
\newcommand{\kpvec}{\ensuremath{{{\bf k}^{\prime}}}}
\newcommand{\km}{\ensuremath{{k^{\protect\phantom{\prime}}}}}
\newcommand{\kpm}{\ensuremath{{k^{\prime}}}}
\newcommand{\kmax}{k_{\rm max}}

% MISC
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\ts}{\textstyle}
\newcommand{\wt}{\widetilde}
%\newcommand{\openone}{\leavevmode\hbox{\small1\normalsize\kern-.33em1}}



